North America Bixby Speaker Diarization System for the VoxCeleb Speaker Recognition Challenge 2021

This paper describes the submission to the speaker diarization track of VoxCeleb Speaker Recognition Challenge 2021 done by North America Bixby Lab of Samsung Research America. Our speaker diarization system consists of four main components such as overlap speech detection and speech separation, robust speaker embedding extraction, spectral clustering with fused affinity matrix, and leakage filtering-based postprocessing. We evaluated our system on the VoxConverse dataset and the challenge evaluation set, which contain natural conversations of multiple talkers collected from YouTube. Our system obtained 4.46%, 6.39%, and 6.16% of the diarization error rate on the VoxConverse development, test, and the challenge evaluation set, respectively.

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

For text: \\
1. literature review: current teacher student learning and semi-supervised
learning method, summary of upsides and downsides. \\
2. Difficulties of teacher student technique in the wild, not in the lab. It is
proof-of-concept-to-production gap.\\

For experiments:\\
1. Check if SOTA pre-trained models (6 models) are available, and how the
  performance is.\\
2. If performance is not enough to use it, we should implement an accuracy
module(tool) to compensate accuracy.\\
3. Find at least five different domain datasets (catelog numbers) from LDC.\\
4. Collect domine-wise labeled data for the domain classifier model.\\
5. Implement CNN domain classifier.

Another ideas:
1. label technique to improve predictions of teacher models.\\
2. Knowledge Distillation for multiple teacher models.\\


Teacher-student training method~\cite{10.1145/3097983.3098135}
Multiple-domain teacher-student training method~\cite{8682887} 



\begin{figure}
\centering
\includegraphics[width=.9\columnwidth]{plots/archtecture_2}
\caption{Archtecture 2}
\label{fig:arch-2}
\end{figure}

\texttt{Accuracy Calibrator} in \autoref{fig:arch-2} is a module to
programmatically adjust each model accuracy. \todo{add how the module works,
  maybe will be use balloon approach}. By adjusting each model accuracy ,
  word-error-rates (WERs), we can find an optimal and minimum accuracy of each
  teacher model for a student. 


\begin{figure*}
\centering
\includegraphics[width=.9\textwidth]{plots/archtecture_1}
\caption{Archtecture 1}
\label{fig:arch-1}
\end{figure*}

\autoref{fig:arch-1} (a) is a domain classifier (CNN model) trained with
multiple domain datasets, The domain classifier takes multiple application
domain input, and classifies domains of audio input. This classifier is used
to distribute unlabeled data to each teacher model based on domain types, and
select which teacher model is used for label prediction in the component of
prediction dispatcher. \todo{can remove prediction dispatcher.}

\autoref{fig:arch-1} (b) shows our pipeline of semi-supervised teacher student
learning. Each teacher model is trained with a specific domain distributed by
the pre-trained domain classifier, and predicts labels for the unlabeled set
for the student model training.

